Are Generative Classifiers More Robust to Adversarial Attacks?

There is a rising interest in studying the robustness of deep neural network classifiers against adversaries, with both advanced attack and defence techniques being actively developed. However, most recent work focuses on discriminative classifiers, which only model the conditional distribution of the labels given the inputs. In this paper, we propose and investigate the deep Bayes classifier, which improves classical naive Bayes with conditional deep generative models. We further develop detection methods for adversarial examples, which reject inputs with low likelihood under the generative model. Experimental results suggest that deep Bayes classifiers are more robust than deep discriminative classifiers, and that the proposed detection methods are effective against many recently proposed attacks.

==> conclusions.tex <==
\section{Discussion}
We have proposed \emph{deep Bayes} as a generative classifier that uses deep latent variable models to model the joint distribution of input-output pairs. Extensive evaluations on multiple classification tasks suggest that generative classifiers are more robust to recently proposed adversarial attacks than discriminative classifiers. Many existing attacks require significantly larger distortions (i.e.~far away from the data manifold) in order to fool the deep Bayes classifier, and at the same time, this increased distortion makes the adversarial images less likely to evade generative model-based detection methods.
%
Our experiments show that modelling unobserved variables is effective for defending against adversarial attacks, which agrees with the Bayesian neural network literature \citep{li:dropout2017, feinman:detecting2017, carlini:bypass2017}.\footnote{In Bayesian neural networks, the network weights are treated as unobserved/latent variables.} But more importantly, the structure of the graphical model has significant impact on robustness, and we show that deep latent variable model-based generative classifiers generally outperform the (randomised) discriminative ones. 
%

We show the robustness of deep Bayes on a binary classification task derived from CIFAR-10, to account for the argument of \citet{carlini:bypass2017} that MNIST properties might not hold on natural images.  We further demonstrate improved robustness on full CIFAR-10 by fusing discriminative visual features and deep Bayes classifiers.
%
Similarly, the k-nearest neighbours classifier, which is closely related to generative classifiers, has also been shown to be robust if deep feature representations are leveraged \citep{papernot:deepknn2018}. Therefore the combination of generative/discriminative models on large-scale real-world datasets is a promising direction for research.

%We do not intend to claim that generative classifiers are robust to \emph{all} possible attacks. On one hand, many recent attacks are designed for discriminative neural networks, while many benchmark datasets have some anti-causal structures \citep{scholkopf:causal2012}. 
%
%On the other hand, naive Bayes as a standard approach for spam filtering is well-known to be fragile \citep{dalvi:adversarial2004,huang:adversarial2011}, and very recently \citet{tabacof:adversarial2016,kos:adversarial2017,creswell:latentpoison2017} also designed attacks for (unconditional) VAE-type models. However, \citet{dalvi:adversarial2004} also showed that generative classifiers can be made more secure if aware of the attack strategy, and \citet{biggio:robustness2011,biggio:security2014} further improved naive Bayes' robustness by modelling the conditional distribution of the adversarial inputs. This is similar to adversarial training deep discriminative classifiers, and efficient ways for doing so with deep Bayes classifiers can be an interesting research direction.

While we have given strong evidence to suggest that generative classifiers are more robust to current adversarial attacks, we do not wish to claim that these models will be robust to \emph{all} possible attacks. Aside from many recent attacks being designed specifically for discriminative neural networks, there is also evidence for the fragility of generative models; e.g. naive Bayes as a standard approach for spam filtering is well-known to be fragile \citep{dalvi:adversarial2004,huang:adversarial2011}, and very recently \citet{tabacof:adversarial2016,kos:adversarial2017,creswell:latentpoison2017} also designed attacks for (unconditional) VAE-type models.
%
%
However, generative classifiers can be made more robust too, to counter these weaknesses. \citet{dalvi:adversarial2004} have shown that generative classifiers can be made more secure if aware of the attack strategy, and \citet{biggio:robustness2011,biggio:security2014} further improved naive Bayes' robustness by modelling the conditional distribution of the adversarial inputs.
These approaches are similar to the adversarial training of discriminative classifiers, and efficient ways for doing so with generative classifiers can be an interesting research direction.

Still, it remains a research challenge to verify the robustness of \emph{fully} generative classifiers on natural images in the wild. Existing deep generative models are less suited for this purpose, indeed PixelCNN-based classifiers perform relatively poorly on CIFAR-10, and, historically, generative classifiers are less accurate than discriminative classifiers at classifying legitimate inputs in high dimensions \citep{efron:efficiency1975, ng:discriminative2002}. Furthermore, training generative classifiers is much more computationally expensive, limiting their current application to  large-scale datasets such as ImageNet. 
%
Therefore, efforts need to be made on developing highly scalable generative models that can capture the data manifold of natural images in a better way. 
%
We believe that progress on this topic can inspire better designs of attack, defence and detection techniques with generative models.
%


==> experiment.tex <==
\section{Experiments}

%
\begin{figure}[t]
\centering
\vspace{-0.2in}
\includegraphics[width=0.98\linewidth]{generative_classifier_iclr/figs/result_white_box_mnist_with_min_dist.pdf}
\vspace{-0.05in}
\caption{Accuracies (column 1), detection rates (columns 2-4) and minimum $\ell_{\inf}$ perturbation (column 6) against \textbf{white-box zero-knowledge} $\ell_{\infty}$ attacks on MNIST. The higher the better. The  second from right most column visualises crafted adversarial examples on an image of digit ``7'', with $\ell_{\infty}$ distortion $\epsilon$ growing from 0.1 to 0.5.}
\vspace{-0.15in}
\label{fig:mnist_white_box}
\end{figure}

We carry out a number of tests on the proposed deep Bayes classifiers (\ref{eq:deep_bayes_vae}), where $q(\z | \cdot)$ and $p(\z | \cdot)$ are factorised Gaussians, and the conditional probability $p(\x | \cdot)$, if required, is parameterised by an $\ell_2$ loss. 
%
Besides the LVM-based classifiers, we further train a Bayesian neural network (BNN) with Bernoulli dropout (dropout rate 0.3), as it has been shown in \citet{li:dropout2017} and \citet{feinman:detecting2017} that BNNs are more robust than their deterministic counterparts. The constructed BNN has 2x more channels than LVM-based classifiers, making the comparison slightly ``unfair'', as the BNN layers have more capacity. We use $K=10$ Monte Carlo samples for all the classifiers.

The adversarial attacks in test include both $\ell_{\infty}$ and $\ell_2$ untargeted attacks from CleverHans 2.0 library \citep{papernot:cleverhans2017}: fast gradient sign method \citep[FGSM,][]{goodfellow:explaining2014}, projected gradient descent \citep[PGD,][]{madry:towards2018}, momentum iterative attack \citep[MIM,][]{dong:mim2017} and Carlini \& Wagner $\ell_2$ \citep[CW,][]{carlini:attack2017}.
%
Two metrics are reported: \emph{accuracy} of the classifier on crafted adversarial examples, and \emph{detection rate} on adversarial examples that have successfully caused the classifier to misclassify. This detection rate is defined as the true positive (TP) rate of finding an adversarial example, and the detection threshold is selected to achieve a $5\%$ false positive rate on clean training data.
%

The experiments are performed under various threat model settings. Due to page limit we only present white-box attacks and gradient masking checks in the main text, and provide a brief summary of further experiments presented in the appendix. Full table results can also be found in the appendix. 
%

\subsection{MNIST}
The first set of experiments evaluate the robustness of generative classifiers on MNIST. Here the image pixel values are normalised to $[0, 1]$, and the LVM-based classifiers have $\text{dim}(\z) = 64$. We first perform white-box \emph{zero-knowledge} attacks, i.e.~the attacker can differentiate through the classifier to craft adversarial examples, but is not aware of the existence of the detector. 
%
Then we perform white-box \emph{perfect-knowledge} attacks, where the attacker can differentiate through both the classifier and the detector, and knows the usage of random $\z$ samples by the VAE-based classifiers \citep{biggio2013evasion, carlini:bypass2017}.
%
Lastly we consider grey-box and black-box attacks, and evaluate the robustness of generative classifiers against transferred attacks.

\paragraph{White-box attacks (zero-knowledge, $\ell_{\infty}$)}
%
%

%
Results for $\ell_{\infty}$ attacks are reported in Figure \ref{fig:mnist_white_box}, and in general generative classifiers perform better in terms of victim accuracy and minimum perturbation of the attacks.\footnote{The minimum perturbation is computed across all $\epsilon$ settings. If none of the attack is successful on an input, we manually assign the minimum perturbation of that input as $\epsilon_{\text{max}} + 0.1$ (0.6 for MNIST).}
%
By contrast, \ref{eq:dfx} \& \ref{eq:dfz} are not robust to the weakest attack (FGSM) even when $\epsilon = 0.2$ (where the adversarial examples are still visually close to the original digit ``7''). Interestingly, \ref{eq:dbx} is the most robust against FGSM \& MIM\footnote{Note that MIM on DBX with $\epsilon=0.9$ achieves $100\%$ success rate (i.e.~victim accuracy $0\%$).}, which agrees with the preliminary tests in \citet{alemi:deepvib2017}. But \ref{eq:dbx} is less robust to PGD, and here \ref{eq:gbz} is a clear winner. These results show that the bottleneck is sometimes beneficial for better robustness of MNIST classifiers. 

For detection, generative classifiers have successfully detected the adversarial examples with $\epsilon \geq 0.3$, which is reasonable as the visual distortion is already significant.
%
Importantly, generative classifier's victim accuracy decreases as the $\ell_{\infty}$ distortion $\epsilon$ increases, but at the same time the TP rates for marginal and logit detection also increase. Therefore these $\ell_{\infty}$ attacks fail to find near-manifold adversarial examples that fool both the classifier and the detection methods.
%
 \ref{eq:dfz}, as an intermediate between generative and discriminative classifiers, has worse robustness results, but has good detection performance for the marginal and logit metrics. This is because with softmax activation, the marginal distribution $p(\x)$ is dropped, but in marginal/logit detection $p(\x)$ is still in use.

%%% CW %%%
\paragraph{White-box attack (zero-knowledge, $\ell_{2}$)}

For the CW $\ell_2$ attack, we performed a hyper-parameter search for the loss-balancing parameter $c$ ($\ell_2$ distortion increases with larger $c$) in $\{0.1, 1, 10, 100, 1000 \}$ on the first 100 test images, and we found $c = 10$ returns the highest success rate. Results are reported in Table \ref{tab:cw_l2_cnn_untargeted}. Although being successful on fooling many classifiers, CW failed on attacking \ref{eq:gbz}. Also, the mean $\ell_2$ distortions of the successful attacks on generative classifiers are significantly larger.
%
Furthermore, we found the success of the attack on other generative classifiers is mainly due to the ambiguity of the crafted adversarial images. As visualised in Figure \ref{fig:cw_attack_input} (also see Figure \ref{fig:cw_attack_appendix} in appendix), the induced distortion from CW leads to ambiguous digits which sit at the perceptual boundary between the original and the adversarial classes.
%
With the KL detection method, all classifiers achieve $> 95\%$ detection rates, which is as expected as the default CW attack configuration, by construction, generates adversarial examples that lead to minimal difference between the logit values of the most and the second most probable classes. 

\input{tables/cw_mnist_vae}

\paragraph{Sanity checks on gradient masking}
%
\citet{athalye:obfuscated2018} claimed that if a successful defence against white-box attacks is due to gradient masking, then this defence is likely to be less effective against grey-box/black-box attacks, as they do not differentiate through the victim classifier and the defence mechanism \citep{papernot:practical2017}.
%
Therefore, we consider two transfer attacks based on distilling the victim classifier using a ``student'' CNN which has no gradient masking. The two attacks differ in their threat models: in the \textbf{grey-box} setting the attacker has access to the output probability vectors of the classifiers on the training data, while in the \textbf{black-box} setting the attacker has access to queried labels only. For the latter black-box setting, we follow \citet{papernot:practical2017} to train a substitute CNN using Jacobian-based dataset augmentation, and we refer to appendix \ref{sec:appendix_black_box_distillation_algorithm} for the detailed algorithm. The grey-box substitutes achieve $>99\%$ agreement with the victims on test data, and the black-box substitutes obtained $\sim 96\%$ accuracy on test data.

Figure \ref{fig:mnist_grey_black_box} shows the accuracy and detection metrics on transferred $\ell_{\infty}$ attacks crafted on the substitute models, with a comparison to their white-box counterparts. Note that these crafted attacks achieve $\sim 100\%$ success rates on fooling the \emph{substitute models} when $\epsilon \geq 0.2$ (see appendix E). However, they do not transfer very well to the generative classifiers. Importantly, for a fixed $\epsilon$ setting, the white-box attacks achieve significantly higher success rates (i.e.~lower victim accuracies) than their grey-/black-box counterparts, and the gap is at least $>20\%$ for $\epsilon \leq 0.3$ (see Table \ref{table:mnist_min_dist}). 
%
We further present the mean minimum $\ell_{\infty}$ perturbation in Table \ref{table:mnist_min_dist}, and we see that the minimum perturbation obtained by grey-/black-box attacks are significantly higher than those obtained by white-box attacks.

All these results suggest that the robustness of generative  classifiers is unlikely to be caused by gradient masking. Again on the detection side, the detection rates increase as the perturbation size increase, and they are near $100\%$ for $\epsilon = 0.3$. This means that most of the successfully transferred adversarial images are off the generative classifier's manifold (as a proxy to the data manifold).

\begin{figure}
%
\vspace{-0.1in}
\centering
\includegraphics[width=1.0\linewidth]{generative_classifier_iclr/figs/result_gradient_masking_mnist_gen_only.pdf}
\vspace{-0.25in}
\captionof{figure}{Accuracy and detection rates against \textbf{distillation-based} attacks on MNIST. The higher the better. We only present generative classifiers' results here, for full results see appendix \ref{sec:appendix_full_results}.}
\label{fig:mnist_grey_black_box}
\vspace{-0.15in}
%
\end{figure}

\input{generative_classifier_iclr/tables/mnist_min_dist.tex}


\paragraph{SPSA (evolutionary strategies)}
We consider another black-box setting that only assumes access to the logit values of the prediction given an input. We use the SPSA $\ell_{\infty}$ attack \citep{uesato:spsa2018}, which is similar to the white-box zero-knowledge attacks, except that gradients are numerically estimated using the logit values from the victim classifier. Results in Table \ref{tab:spsa_mnist} clearly show that SPSA performs much worse on generative classifiers when compared to \emph{white-box} PGD. Again this means gradient masking is unlikely to be responsible for the improved robustness of generative classifiers, as utilising the exact gradient yielded improved results. 
%

\begin{figure}
\centering
\vspace{-0.2in}
\captionof{table}{Accuracy and detection rates against  \textbf{black-box SPSA attack} ($\epsilon=0.3$), with a comparison to white-box PGD on 1000 randomly sampled test datapoints. The higher the better.}
\vspace{-0.1in}
\centering
\label{tab:spsa_mnist}
\begin{tabular}{c|cccc|ccc}\toprule 
  & GFZ & GBZ & GBY & GFY & DFX & DBX & DFZ \\
  \toprule
  PGD victim acc & 4.0\% & 29.7\% & 7.4\% & 2.3\% & 0.0\% & 5.4\% & 0.0\% \\
  \midrule
  SPSA victim acc & 68.2\% & 79.0\% & 71.0\% & 55.9\% & 0.0\% & 46.3\% & 11.0\% \\
  SPSA TP logit & 91.5\% & 92.4\% & 95.7\% & 98.5\% & N/A & N/A & 65.8\% \\
\bottomrule 
\end{tabular} 
\end{figure}

%%%%%%%% CIFAR %%%%%%%


\subsection{CIFAR plane-vs-frog binary classification}

We consider the same set of evaluations on CIFAR-10, in order to validate the robustness of generative classifiers on natural images \citep[c.f.][]{carlini:bypass2017}. Unfortunately, we failed to train \emph{fully} generative classifiers with comparable test accuracies to discriminative CNNs (typically $>80\%$): the clean accuracies for \ref{eq:gfz} \& \ref{eq:gfy} are all $<50\%$. Even when using the conditional PixelCNN++ \citep{salimans:pixelcnn++2017} (which uses much deeper networks), the clean accuracy on the test data is $72.4\%$. Instead, we consider a simpler binary classification problem and construct a dataset containing CIFAR images from the ``airplane'' and ``frog'' categories. The images in this dataset are scaled to [0, 1]. On this dataset, the generative classifiers use $\text{dim}(\z) = 128$ and obtain $>90\%$ clean test accuracy (see appendix). The attacks are performed on the test images that all models initially correctly classify, leading to a test set of 1577 instances. Due to the page limit, we only present white-box zero-knowledge attacks here, and discuss further attacks in the appendix.

\paragraph{White-box attacks (zero-knowledge, $\ell_{\infty}$)}
We present the white-box $\ell_{\infty}$ attack results in Figure \ref{fig:cifar_white_box}, where the distortion strengths are selected as $\epsilon \in \{0.01, 0.02, 0.05, 0.1, 0.2 \}$. Again, generative classifiers are more robust than the discriminative ones, and \ref{eq:gbz} is the most robust, much better than the others when $\epsilon \geq 0.05$. BNN is significantly better than other discriminative VAE-based classifiers, presumably due to higher randomness. Detection results are less satisfactory: marginal/logit detection fail to detect attacks with $\epsilon = 0.1$ (which attain both high success rate and induce visually perceptible distortion). KL detection performs better, and interestingly, discriminative classifiers dominate in this metric. These results suggest that the $\ell_2$ likelihood might not be best suited for modelling natural images \citep[c.f.][]{larsen:vaegan2016, oord:pixel2016}. Still, the minimum distortion required to fool generative classifiers are much higher than that for discriminative ones, indeed the visual distortion of the adversarial examples on generative classifiers are more significant.


\paragraph{White-box attack (zero-knowledge, $\ell_{2}$)}
As the test set is relatively small, we directly perform CW attacks on the test data with $c \in \{0.1, 1, 10, 100, 1000\}$. Results are visualised in Figure \ref{fig:cifar_white_box_cw}. The generative classifiers are significantly more robust than the others (with the best being \ref{eq:gbz}), and the mean $\ell_2$ distortions computed on successful attacks are also significantly higher. The TP rates are low for marginal and logit detection, which is reasonable as the crafted images are visually similar to the clean ones. Note that the distortion for the attacks on generative classifiers is perceptible. These results indicate that this CW attack is ineffective when attacking generative classifiers.

\begin{figure}
\centering
\vspace{-0.2in}
\includegraphics[width=0.98\linewidth]{figs/result_white_box_plane_frog_with_min_dist.pdf}
\vspace{-0.05in}
\caption{Accuracy, detection rates and minimum $\ell_{\inf}$ perturbations against \textbf{white-box zero-knowledge} $\ell_{\infty}$ attacks on the CIFAR plane-vs-frog dataset. The higher the better. The second from right most column visualises crafted adversarial examples on an image of a plane, with $\ell_{\infty}$ distortion $\epsilon \in \{0.01, 0.02, 0.05, 0.1, 0.2 \}$.}
\vspace{-0.1in}
\label{fig:cifar_white_box}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{figs/result_cw_plane_frog.pdf}
\vspace{-0.1in}
\caption{Accuracy and detection rates against \textbf{white-box zero-knowledge} CW attacks on the CIFAR plane-vs-frog dataset. The higher the better.}
\vspace{-0.1in}
\label{fig:cifar_white_box_cw}
\end{figure}

\subsection{Full CIFAR-10: combining deep Bayes and discriminative features}

The final experiment examines the robustness of CIFAR-10 \emph{multi-class} classifiers, with the generative classifiers trained on \emph{discriminative} visual features. To do this, we download a pretrained deep convolutional net\footnote{\url{https://github.com/geifmany/cifar-vgg}, $93.59\%$ test accuracy} with VGG16-like architecture \citep{simonyan2014very}, and use its feature representation $\bm{\phi}(\x)$ as the input to the VAE-based classifiers: $p(\y|\x) = p(\y | \bm{\phi}(\x))$. 
%
The classifiers in test include \ref{eq:gbz}, \ref{eq:gby} and \ref{eq:dbx}. We use fully-connected neural networks for these classifiers, and select from VGG16 the $9^{\text{th}}$ convolution layer (\textsc{conv9}) and the first fully connected layer after convolution (\textsc{fc1}) as the feature layers to ensure $\sim 90\%$ test accuracy (see appendix).

Results on \textbf{white-box zero-knowledge $\ell_{\infty}$ attacks} are  visualised in Figure \ref{fig:vgg_white_box}. Compared with the VGG16 baseline, we see clear improvements in robustness and detection for all VAE-based classifiers. In particular, the generative classifiers \ref{eq:gbz} and \ref{eq:gby} are overall better than \ref{eq:dbx}. More importantly, generative classifiers based on \textsc{conv9} features are significantly more robust than those based on \textsc{fc1} features. In contrast, for \ref{eq:dbx}, which is \emph{discriminative}, the robustness results are very similar, indicating that the level of feature representation has little effect. These results suggest that one can achieve both high clean accuracy and better robustness against adversaries by combining discriminatively learned visual features and generative classifiers.

\begin{figure}
\centering
\includegraphics[width=1.\linewidth]{figs/result_fea_cifar10.pdf}
\vspace{-0.2in}
\caption{Accuracy and detection rates against \textbf{white-box zero-knowledge} $\ell_{\infty}$ attacks on CIFAR-10. The higher the better. Note that results for the DBX classifiers are almost identical.}
\vspace{-0.15in}
\label{fig:vgg_white_box}
\end{figure}

\subsection{Further experiments}
In the appendix we present extra experiments to compare the robustness properties of generative/discriminative classifiers. In below we provide a brief summary of the observations there, readers are referred to the appendix for further details.
\begin{itemize}
    \item white-box perfect knowledge attack
    \item Bottleneck effect
    \item distillation based attack
    \item cross-model transfer
\end{itemize}


==> tables/cw_mnist_vae.tex <==
\begin{figure}
%
\captionof{table}{\textbf{White-box} CW-$\ell_2$ attack results. Here, accuracy (adv) measures classifying the adversarial inputs to the original classes.}
\centering
\label{tab:cw_l2_cnn_untargeted}
\scalebox{0.85}{
\begin{tabular}{c|cccc}
\hline 
  & acc.~(clean) & acc.~(adv) & $\ell_2$ dist. & TP KL\\
  \hline
BNN  & $99.12\%$ & $24.40\%$ & $2.129$ & $95.31$ \\
\ref{eq:gfz} & $98.55\%$ & $28.58\%$ & $2.663$ & $95.37$ \\
\ref{eq:gbz} & $97.45\%$ & $81.51\%$ & $2.446$ & $91.01$ \\
\ref{eq:gfy} & $99.15\%$ & $28.64\%$ & $2.732$ & $96.03$ \\
\ref{eq:gby} & $98.72\%$ & $32.72\%$ & $2.735$ & $94.46$ \\
\ref{eq:dfx} & $99.10\%$ & $20.31\%$ & $2.095$ & $99.96$\\
\ref{eq:dbx} & $98.87\%$ & $30.19\%$ & $1.806$ & $96.76$ \\
\ref{eq:dfz} & $99.10\%$ & $13.60\%$ & $2.188$ & $99.57$ \\
\hline 
\end{tabular} 
}

%
\hspace{2em}
%
\vspace{-1em}
\subfigure[clean inputs]{
\includegraphics[width=0.35\linewidth]{figs/data_clean.png}}
\hspace{0.1in}
%
\subfigure[CW adv.~inputs]{
\includegraphics[width=0.35\linewidth]{figs/bayes_A_cw_adv_annotated.png}}
\captionof{figure}{Visualising the clean inputs and the CW adversarial examples crafted on \ref{eq:gfz}, digits in red rectangles show significant ambiguity.}
\label{fig:cw_attack_input}
\vspace{-0.1in}
\end{figure}

==> tables/spsa_mnist.tex <==
\begin{table}[!h]
\caption{Accuracy against SPSA attack (with a comparision to white-box PGD).}
\centering
\label{tab:spsa_mnist}
\begin{tabular}{c|ccccccc}\hline 
  & GFZ & GBZ & GBY & GFY & DFX & DBX & DFZ \\
  PGD & A & B & C & D & E & F & G \\
  SPSA & A & B & C & D & E & F & G \\
\hline 
\end{tabular} 
\end{table}

==> tables/tables_grey_box/cw_mnist.tex <==
\begin{table}
\caption{Grey-box CW attack results on MNIST. }
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc|ccccc|ccccc}\hline
 & \multicolumn{5}{c|}{substitute acc} & \multicolumn{5}{c|}{victim acc} & \multicolumn{5}{c|}{TP logit} \\
\hline
$c$ & 0.10 & 1.00 & 10.00 & 100.00 & 1000.00 & 0.10 & 1.00 & 10.00 & 100.00 & 1000.00 & 0.10 & 1.00 & 10.00 & 100.00 & 1000.00 \\
\hline
GFZ & $ 98.4 $ &$ 4.6 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 98.9 $ &$ 96.8 $ &$ 96.0 $ &$ 93.6 $ &$ 90.3 $ &$ 50.9 $ &$ 41.3 $ &$ 40.7 $ &$ 36.2 $ &$ 39.1 $  \\
GBZ & $ 98.4 $ &$ 63.2 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 97.5 $ &$ 95.4 $ &$ 93.0 $ &$ 89.0 $ &$ 84.4 $ &$ 47.9 $ &$ 39.9 $ &$ 31.7 $ &$ 30.3 $ &$ 36.9 $  \\
GFY & $ 98.1 $ &$ 0.9 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 99.0 $ &$ 97.6 $ &$ 97.0 $ &$ 95.9 $ &$ 94.2 $ &$ 54.0 $ &$ 42.6 $ &$ 43.1 $ &$ 42.3 $ &$ 48.2 $  \\
GBY & $ 98.3 $ &$ 5.3 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 98.7 $ &$ 97.0 $ &$ 96.2 $ &$ 93.6 $ &$ 90.8 $ &$ 45.8 $ &$ 38.4 $ &$ 35.2 $ &$ 37.4 $ &$ 42.9 $  \\
DFX & $ 85.1 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 97.6 $ &$ 93.3 $ &$ 91.2 $ &$ 90.4 $ &$ 89.8 $ & N/A & N/A & N/A & N/A & N/A  \\
DBX & $ 97.3 $ &$ 46.0 $ &$ 0.4 $ &$ 0.0 $ &$ 0.0 $ &$ 98.7 $ &$ 93.9 $ &$ 88.4 $ &$ 85.5 $ &$ 76.3 $ & N/A & N/A & N/A & N/A & N/A  \\
DFZ & $ 80.5 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 97.4 $ &$ 94.4 $ &$ 92.2 $ &$ 91.7 $ &$ 91.1 $ &$ 27.0 $ &$ 22.5 $ &$ 22.1 $ &$ 32.2 $ &$ 38.8 $  \\
\hline
\end{tabular}
\end{table}


==> tables/tables_grey_box/cw_plane_frog.tex <==
\begin{table}
\caption{Grey-box CW attack results on CIFAR plane-vs-frog binary classification. }
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc|ccccc|ccccc}\hline
 & \multicolumn{5}{c|}{substitute acc} & \multicolumn{5}{c|}{victim acc} & \multicolumn{5}{c|}{TP logit} \\
\hline
$c$ & 0.10 & 1.00 & 10.00 & 100.00 & 1000.00 & 0.10 & 1.00 & 10.00 & 100.00 & 1000.00 & 0.10 & 1.00 & 10.00 & 100.00 & 1000.00 \\
\hline
GFZ & $ 98.7 $ &$ 61.9 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 98.9 $ &$ 95.9 $ &$ 94.9 $ &$ 94.5 $ &$ 93.3 $ &$ 10.0 $ &$ 2.1 $ &$ 4.5 $ &$ 4.1 $ &$ 4.1 $  \\
GBZ & $ 96.3 $ &$ 69.8 $ &$ 3.3 $ &$ 0.0 $ &$ 0.0 $ &$ 95.3 $ &$ 94.9 $ &$ 93.6 $ &$ 93.5 $ &$ 93.5 $ &$ 18.2 $ &$ 16.9 $ &$ 17.9 $ &$ 17.3 $ &$ 17.3 $  \\
GFY & $ 98.4 $ &$ 54.4 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 98.4 $ &$ 95.9 $ &$ 95.0 $ &$ 94.9 $ &$ 94.2 $ &$ 13.0 $ &$ 5.5 $ &$ 4.1 $ &$ 5.0 $ &$ 4.4 $  \\
GBY & $ 97.6 $ &$ 52.9 $ &$ 2.2 $ &$ 0.0 $ &$ 0.0 $ &$ 97.9 $ &$ 95.1 $ &$ 94.1 $ &$ 93.8 $ &$ 93.3 $ &$ 20.9 $ &$ 13.0 $ &$ 11.1 $ &$ 13.1 $ &$ 16.2 $  \\
DFX & $ 64.4 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 98.5 $ &$ 97.2 $ &$ 97.1 $ &$ 96.7 $ &$ 95.5 $ & N/A & N/A & N/A & N/A & N/A  \\
DBX & $ 91.3 $ &$ 56.2 $ &$ 0.3 $ &$ 0.0 $ &$ 0.0 $ &$ 99.7 $ &$ 99.0 $ &$ 99.0 $ &$ 98.9 $ &$ 98.1 $ & N/A & N/A & N/A & N/A & N/A  \\
DFZ & $ 80.3 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 98.9 $ &$ 97.7 $ &$ 97.5 $ &$ 97.5 $ &$ 95.9 $ &$ 0.0 $ &$ 24.5 $ &$ 20.6 $ &$ 15.4 $ &$ 13.2 $  \\
\hline
\end{tabular}
\end{table}


==> tables/tables_grey_box/mim_mnist.tex <==
\begin{table}
\caption{Grey-box MIM attack results on MNIST. }
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc|ccccc|ccccc}\hline
 & \multicolumn{5}{c|}{substitute acc} & \multicolumn{5}{c|}{victim acc} & \multicolumn{5}{c|}{TP logit} \\
\hline
$\epsilon$ & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 \\
\hline
GFZ & $ 87.6 $ &$ 24.6 $ &$ 1.1 $ &$ 0.3 $ &$ 0.3 $ &$ 96.2 $ &$ 82.1 $ &$ 44.1 $ &$ 16.8 $ &$ 16.8 $ &$ 46.5 $ &$ 79.5 $ &$ 99.9 $ &$ 100.0 $ &$ 100.0 $  \\
GBZ & $ 81.8 $ &$ 9.1 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 93.6 $ &$ 79.0 $ &$ 45.6 $ &$ 17.4 $ &$ 5.1 $ &$ 42.6 $ &$ 81.3 $ &$ 100.0 $ &$ 100.0 $ &$ 100.0 $  \\
GFY & $ 85.9 $ &$ 14.2 $ &$ 0.8 $ &$ 0.2 $ &$ 0.2 $ &$ 96.6 $ &$ 80.6 $ &$ 49.5 $ &$ 23.4 $ &$ 23.4 $ &$ 56.9 $ &$ 95.1 $ &$ 100.0 $ &$ 100.0 $ &$ 100.0 $  \\
GBY & $ 87.0 $ &$ 15.9 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 96.0 $ &$ 79.7 $ &$ 41.6 $ &$ 13.1 $ &$ 3.9 $ &$ 48.1 $ &$ 86.7 $ &$ 100.0 $ &$ 100.0 $ &$ 100.0 $  \\
DFX & $ 76.5 $ &$ 12.3 $ &$ 3.6 $ &$ 2.1 $ &$ 2.1 $ &$ 91.5 $ &$ 56.1 $ &$ 22.2 $ &$ 9.9 $ &$ 9.9 $ & N/A & N/A & N/A & N/A & N/A  \\
DBX & $ 85.1 $ &$ 19.9 $ &$ 0.6 $ &$ 0.1 $ &$ 0.1 $ &$ 93.4 $ &$ 57.0 $ &$ 14.1 $ &$ 6.3 $ &$ 6.3 $ & N/A & N/A & N/A & N/A & N/A  \\
DFZ & $ 72.3 $ &$ 7.4 $ &$ 1.4 $ &$ 0.8 $ &$ 0.8 $ &$ 91.7 $ &$ 56.4 $ &$ 20.9 $ &$ 8.4 $ &$ 8.4 $ &$ 32.3 $ &$ 63.3 $ &$ 98.9 $ &$ 100.0 $ &$ 100.0 $  \\
\hline
\end{tabular}
\end{table}


==> tables/tables_grey_box/mim_plane_frog.tex <==
\begin{table}
\caption{Grey-box MIM attack results on CIFAR plane-vs-frog binary classification. }
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc|ccccc|ccccc}\hline
 & \multicolumn{5}{c|}{substitute acc} & \multicolumn{5}{c|}{victim acc} & \multicolumn{5}{c|}{TP logit} \\
\hline
$\epsilon$ & 0.01 & 0.02 & 0.05 & 0.10 & 0.20 & 0.01 & 0.02 & 0.05 & 0.10 & 0.20 & 0.01 & 0.02 & 0.05 & 0.10 & 0.20 \\
\hline
GFZ & $ 96.3 $ &$ 87.9 $ &$ 42.1 $ &$ 4.7 $ &$ 0.1 $ &$ 97.9 $ &$ 95.5 $ &$ 83.3 $ &$ 46.5 $ &$ 5.8 $ &$ 3.8 $ &$ 5.5 $ &$ 4.6 $ &$ 8.4 $ &$ 76.3 $  \\
GBZ & $ 92.9 $ &$ 82.5 $ &$ 36.9 $ &$ 4.9 $ &$ 0.0 $ &$ 94.5 $ &$ 93.6 $ &$ 90.2 $ &$ 80.7 $ &$ 51.1 $ &$ 17.1 $ &$ 16.6 $ &$ 16.0 $ &$ 21.8 $ &$ 98.0 $  \\
GFY & $ 96.8 $ &$ 87.9 $ &$ 34.1 $ &$ 3.5 $ &$ 0.1 $ &$ 97.1 $ &$ 95.3 $ &$ 84.4 $ &$ 49.9 $ &$ 7.4 $ &$ 7.2 $ &$ 5.4 $ &$ 6.6 $ &$ 10.4 $ &$ 81.2 $  \\
GBY & $ 95.1 $ &$ 85.5 $ &$ 32.0 $ &$ 2.6 $ &$ 0.1 $ &$ 96.4 $ &$ 94.8 $ &$ 85.9 $ &$ 54.4 $ &$ 10.7 $ &$ 16.9 $ &$ 13.9 $ &$ 8.4 $ &$ 13.7 $ &$ 97.6 $  \\
DFX & $ 95.5 $ &$ 80.5 $ &$ 10.5 $ &$ 0.2 $ &$ 0.0 $ &$ 99.1 $ &$ 96.5 $ &$ 77.3 $ &$ 24.0 $ &$ 0.2 $ & N/A & N/A & N/A & N/A & N/A  \\
DBX & $ 95.6 $ &$ 81.1 $ &$ 34.5 $ &$ 2.2 $ &$ 0.0 $ &$ 99.5 $ &$ 98.3 $ &$ 89.3 $ &$ 58.9 $ &$ 9.9 $ & N/A & N/A & N/A & N/A & N/A  \\
DFZ & $ 96.3 $ &$ 81.5 $ &$ 10.7 $ &$ 0.5 $ &$ 0.0 $ &$ 99.1 $ &$ 96.5 $ &$ 74.9 $ &$ 21.7 $ &$ 0.3 $ &$ 0.0 $ &$ 7.3 $ &$ 6.4 $ &$ 10.3 $ &$ 80.8 $  \\
\hline
\end{tabular}
\end{table}


==> tables/tables_grey_box/pgd_mnist.tex <==
\begin{table}
\caption{Grey-box PGD attack results on MNIST. }
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc|ccccc|ccccc}\hline
 & \multicolumn{5}{c|}{substitute acc} & \multicolumn{5}{c|}{victim acc} & \multicolumn{5}{c|}{TP logit} \\
\hline
$\epsilon$ & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 \\
\hline
GFZ & $ 86.8 $ &$ 14.5 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 96.2 $ &$ 83.5 $ &$ 52.0 $ &$ 27.1 $ &$ 17.2 $ &$ 47.1 $ &$ 74.0 $ &$ 99.8 $ &$ 100.0 $ &$ 100.0 $  \\
GBZ & $ 81.2 $ &$ 9.1 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 93.8 $ &$ 80.4 $ &$ 56.9 $ &$ 34.4 $ &$ 25.5 $ &$ 44.4 $ &$ 72.9 $ &$ 99.6 $ &$ 100.0 $ &$ 100.0 $  \\
GFY & $ 84.9 $ &$ 6.5 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 96.7 $ &$ 82.3 $ &$ 54.9 $ &$ 33.4 $ &$ 24.2 $ &$ 54.4 $ &$ 89.0 $ &$ 100.0 $ &$ 100.0 $ &$ 100.0 $  \\
GBY & $ 86.7 $ &$ 15.0 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 95.9 $ &$ 81.3 $ &$ 50.4 $ &$ 27.2 $ &$ 18.4 $ &$ 47.1 $ &$ 78.7 $ &$ 99.9 $ &$ 100.0 $ &$ 100.0 $  \\
DFX & $ 74.2 $ &$ 5.2 $ &$ 0.5 $ &$ 0.0 $ &$ 0.0 $ &$ 91.7 $ &$ 57.7 $ &$ 19.6 $ &$ 4.3 $ &$ 1.4 $ & N/A & N/A & N/A & N/A & N/A  \\
DBX & $ 80.6 $ &$ 5.1 $ &$ 0.0 $ &$ 0.0 $ &$ 0.0 $ &$ 93.2 $ &$ 59.2 $ &$ 22.5 $ &$ 10.9 $ &$ 8.2 $ & N/A & N/A & N/A & N/A & N/A  \\
DFZ & $ 69.5 $ &$ 3.5 $ &$ 0.2 $ &$ 0.0 $ &$ 0.0 $ &$ 92.0 $ &$ 56.9 $ &$ 21.5 $ &$ 6.8 $ &$ 2.9 $ &$ 30.5 $ &$ 53.8 $ &$ 91.7 $ &$ 100.0 $ &$ 100.0 $  \\
\hline
\end{tabular}
\end{table}


==> tables/tables_grey_box/pgd_plane_frog.tex <==
\begin{table}
\caption{Grey-box PGD attack results on CIFAR plane-vs-frog binary classification. }
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc|ccccc|ccccc}\hline
 & \multicolumn{5}{c|}{substitute acc} & \multicolumn{5}{c|}{victim acc} & \multicolumn{5}{c|}{TP logit} \\
\hline
$\epsilon$ & 0.01 & 0.02 & 0.05 & 0.10 & 0.20 & 0.01 & 0.02 & 0.05 & 0.10 & 0.20 & 0.01 & 0.02 & 0.05 & 0.10 & 0.20 \\
\hline
GFZ & $ 96.7 $ &$ 88.1 $ &$ 41.7 $ &$ 4.5 $ &$ 0.1 $ &$ 97.9 $ &$ 95.5 $ &$ 84.1 $ &$ 48.8 $ &$ 9.3 $ &$ 3.8 $ &$ 5.6 $ &$ 4.0 $ &$ 7.4 $ &$ 51.4 $  \\
GBZ & $ 92.9 $ &$ 83.1 $ &$ 37.8 $ &$ 5.5 $ &$ 0.0 $ &$ 94.6 $ &$ 93.5 $ &$ 90.3 $ &$ 82.9 $ &$ 65.6 $ &$ 17.9 $ &$ 17.6 $ &$ 15.2 $ &$ 20.7 $ &$ 80.6 $  \\
GFY & $ 96.9 $ &$ 88.1 $ &$ 33.7 $ &$ 3.3 $ &$ 0.1 $ &$ 97.2 $ &$ 95.4 $ &$ 85.3 $ &$ 54.9 $ &$ 13.3 $ &$ 7.3 $ &$ 5.5 $ &$ 6.5 $ &$ 8.3 $ &$ 61.8 $  \\
GBY & $ 95.2 $ &$ 85.6 $ &$ 32.4 $ &$ 2.8 $ &$ 0.1 $ &$ 96.4 $ &$ 94.8 $ &$ 86.4 $ &$ 59.1 $ &$ 17.5 $ &$ 16.9 $ &$ 13.9 $ &$ 8.6 $ &$ 11.9 $ &$ 74.3 $  \\
DFX & $ 95.7 $ &$ 80.8 $ &$ 10.1 $ &$ 0.2 $ &$ 0.0 $ &$ 99.1 $ &$ 96.7 $ &$ 79.4 $ &$ 28.3 $ &$ 0.9 $ & N/A & N/A & N/A & N/A & N/A  \\
DBX & $ 95.7 $ &$ 80.5 $ &$ 30.5 $ &$ 1.7 $ &$ 0.0 $ &$ 99.5 $ &$ 98.2 $ &$ 91.1 $ &$ 65.1 $ &$ 21.8 $ & N/A & N/A & N/A & N/A & N/A  \\
DFZ & $ 96.5 $ &$ 81.9 $ &$ 10.5 $ &$ 0.3 $ &$ 0.0 $ &$ 99.1 $ &$ 97.1 $ &$ 77.6 $ &$ 25.5 $ &$ 1.3 $ &$ 0.0 $ &$ 5.5 $ &$ 6.7 $ &$ 9.3 $ &$ 60.0 $  \\
\hline
\end{tabular}
\end{table}

